Demonstration of Machine Learning-assisted real-time noise regression in gravitational wave detectors

Real-time noise regression algorithms are crucial for maximizing the science outcomes of the LIGO, Virgo, and KAGRA gravitational-wave detectors. This includes improvements in the detectability, source localization and pre-merger detectability of signals thereby enabling rapid multi-messenger follow-up. In this paper, we demonstrate the effectiveness of \textit{DeepClean}, a convolutional neural network architecture that uses witness sensors to estimate and subtract non-linear and non-stationary noise from gravitational-wave strain data. Our study uses LIGO data from the third observing run with injected compact binary signals. As a demonstration, we use \textit{DeepClean} to subtract the noise at 60 Hz due to the power mains and their sidebands arising from non-linear coupling with other instrumental noise sources. Our parameter estimation study on the injected signals shows that \textit{DeepClean} does not do any harm to the underlying astrophysical signals in the data while it can enhances the signal-to-noise ratio of potential signals. We show that \textit{DeepClean} can be used for low-latency noise regression to produce cleaned output data at latencies $\sim 1-2$\, s. We also discuss various considerations that may be made while training \textit{DeepClean} for low latency applications.

==> sec-MDC.tex <==
\section{A Mock Data Challenge}\label{sec-MDC}

To evaluate the effectiveness of \textit{DeepClean}, we performed an end-to-end analysis of mock data through a Mock Data challenge (MDC) introduced by the LVK to benchmark and prepare the low latency analysis pipelines. The mock data is generated by injecting compact binary signals into the O3 strain data from LIGO Hanford and LIGO Livingston. We selected the low-latency O3 data (labeled as \verb|GDS-CALIB_STRAIN|) from the 20-day period between September 1, 00:00:00 UTC and September 20, 00:00:00 UTC.% chosen based on a coherence study presented in Appendix \ref{sec:coherence}. 
This period exhibits high coherence between the strain and intended witness channels %(which are discussed in detail later) 
in both H1 and L1, making it well-suited for testing the performance of \textit{DeepClean}.

The injected compact binary signals comprise binary black hole mergers, binary neutron star mergers, and neutron star-black hole mergers. The parameters of the injections such as masses, spins, luminosity distance, and other extrinsic parameters, are drawn from simulated distributions that are consistent with the O3-inferred population models~\cite{GWTC3pop} %(see Appendix \ref{sec-mdc-appendix} for more information).
The coalescence times of the 25,000 injections are uniformly distributed over the 20--day period, such that there are no overlapping signals. Additionally, all the signals are generated by using 10\,Hz as the  lower cut-off frequency.

%This injection sets we used are the same as injections used by the \textit{LIGO MDC} that was generated and used for testing the readiness of various analysis pipelines for O4. While the LIGO MDC injects 50000 signals over 40 days period, we use the first 20-days which means the first 25000 injections, keeping the same injection density.








==> sec-asdr.tex <==

\subsection{Comparison of ASD ratios}



==> sec-coherence.tex <==
\subsection{Coherence estimation between IFO strain and noise witness}\label{sec:coherence}

\begin{figure*}
    \centering
    \includegraphics[scale=0.24]{coherence.png}
    \caption{{\red Actions for Saleem: Need an updated figure in pdf format and standard label sizes. Keep a gap during October when H1L1 were not in operation} Figure showing the coherence between GDS-CALIB\_STRAIN and one of the power-line witness channels, PEM-CS\_MAINSMON\_EBAY\_1\_DQ.  For H1, the MAINSMON channel tracks the powerline amplitude strongly so that the coherence is $\sim 1$ while for L1, a strong coherence is noted only for about two months (2019 Aug-Sept) of the entire O3.}
\label{fig:coherence}
\end{figure*}


The coherence between two time series streams $h(t)$ and $w(t)$ at a given frequency $f$ can be estimated using the following expression \cite{Coughlin:2019hcf},
\begin{equation}
    C(f) =\frac{ \langle \tilde{h}(f) \tilde{w}^*(f) \rangle }{\sqrt{ \langle \vert \tilde{h}(f)\vert^2 \rangle \langle \vert \tilde{w}^*(f) \vert^2 \rangle }},
    \label{eq:coherence}
\end{equation}
where $\tilde{h}(f)$ and $\tilde{w}(f)$ are respectively the Fourier transforms of $h(t)$ and $w(t)$, $^*$ represents the complex conjugate, and $\langle . \rangle$ represents the time average over a number of consecutive time windows. The coherence tracks the relative phase of the two time series streams and will be unity if both the time series are exactly identical. If the two time series streams are correlated to some extend, the coherence $C(f)$
will show a value between 0 and 1 depending on the strength of correlation. 
For a noise witness channel that is coupled to the interferometer strain, the coherence is expected to be high and hence we use coherence as an indicator of whether a witness channel carries useful information about the noise coupling to the $h(t)$. 

In this study, as mentioned earlier, our main subtraction target is the power-line noise at 60 Hz and their sidebands due to the non-linear coupling with other instrumental noise sources such as the noise produced by the alignment sensor setup that control the optics. We computed coherence between the strain channel \verb|GDS-CALIB_STRAIN| and one of the power-line witness channels, \verb|PEM-CS_MAINSMON_EBAY_1_DQ| for entire O3 data from L1 and H1. More precisely, we compute $C$ as in equation~\ref{eq:coherence} for 1\,s frames sampled at 16 kHz and perform the average over 1024 such segments. The analysis is performed at the first and last 1024\,s of every lock stretches - where a lock stretch is the period in which the interferometer is in locked state between the happenings of two lock-losses. 

Figure \ref{fig:coherence} shows the coherence computed for the entire O3 data, as described above. While there is a high ($\sim ~ 1$) coherence between the two channels in LIGO Hanford during the entire O3, the same is not true for the data in LIGO Livingston. A close-to-unity value is observed only during August-September, 2019. While the coherence falls by about 5-20\% during April-July 2019, the value is significantly down and unstable during the second part of O3 (namely O3b, spanning November 2019 - April 2020). 

While deepclean relies on how well the contributors of the coupled noise sources are recorded by the dedicated witness sensors, we found that the subtraction gets affected significantly when the coherence goes below some level. While the coherence pattern found during April-July 2019 of O3a only affected the subtraction of the power-line mildly, those of O3b led to poor subtraction of the power-line and sidebands. It is a future goal to explore how much can we improve the subtraction by fine-tuning the neural network when the coherence goes sub-optimal. 

In the present study, we have used this information as a navigator for the segment selection for our MDC. The first 10 days of September is chosen following the high coherence during that period at both H1 and L1. 
     


==> sec-gstlal.tex <==


\subsection{Compact binary search sensitivity}
%How Gstlal works.

%How we simulate data

\begin{figure}
    \centering
    \includegraphics[scale=0.6]{figures/VT-vs-FAR.png}
    \caption{The fractional improvement in sensitive volume ($VT$) measured by GstLAL (after \textit{DeepClean} to before \textit{DeepClean}) shown as a function of the estimated false-alarm-rate. \textit{DeepClean} improves the sensitive volume of the search for false-alarm-rates of approximately 2 per day to 1 per 100 years, but there is a slight loss in sensitivity to very high significance events. 
    }
    \label{fig:gstlal}
\end{figure}

{\color{black}
The GstLAL-based inspiral pipeline (referred to as GstLAL) is a matched-filtering based pipeline used to detect compact binary mergers~\citep{Sachdev:2019,Hanna:2019ezx,Messick:2017,Tsukada:2023edh,2021SoftX..1400680C}. GstLAL has played an instrumental role in low-latency detections of gravitational-waves~\citep{LIGOScientific:2016sjg,AbEA2017b}, and directly enabled the observation of electromagnetic counterparts associated with a BNS merger~\citep{LIGOScientific:2017ync,G298048}.

We perform two GstLAL analyses on $\sim$\,20 days of O3 data to assess the performance of \textit{DeepClean}. The first analysis acts as a control and uses the final strain frames cleaned and published by Advanced LIGO and Advanced Virgo~\citep{LIGOScientific:2023vdi}. The second analysis ingests the frames processed by \textit{DeepClean}. In each analysis, we search for a set of astrophysically distributed simulated gravitational-wave signals, or \emph{injections}. The injections span $m_i \in [5 M\odot, 50 M\odot]$ in component mass and $s_{i\rm{z}} \in [0, 0.99]$ in component spin aligned with the orbital angular momentum. We evenly space the resulting $54 000$ injections 32\,seconds apart, and separately place them into each data stream. 

We find that we recover more injections in data cleaned by \textit{DeepClean} for false-alarm-rates between 2 per day and 1 per 100 years, as shown in Fig.~\ref{fig:gstlal}. For highly significant simulations (false-alarm-rates less than 1 per 100 years), here is a slight loss in sensitivity. We do not expect that this loss significantly impacts the chance of detection for these loud events. We hypothesize that this behavior is a result of \textit{DeepClean} focusing on removing quiet noise artifacts while leaving loud noise transients from other sources in the data, causing the slope of the extrapolated background to lessen. In the limit of more data, we expect the $VT$ ratio at high significance to asymptote to 1; we leave confirmation of this behavior to future work.


%\ms{Action item for Ryan: text and figure to be added}




==> sec-inference.tex <==

\section{Applying \textit{DeepClean} on the mock data}
\label{sec:inference}

The noise regression analysis is performed in two steps; training and cleaning (also referred to as the \textit{inference}). Below we describe the operational parameters of training and cleaning considered in this study.

\subsection{Strategy for Training and Cleaning the MDC data}

To train and clean the 20 days of MDC data, we adopted a strategy that involves selecting only science-quality data labeled as \verb|DMT-ANALYSIS_READY:1|. In total, we identified 47 science sub-segments (\textit{a.k.a} active segments)\footnote{For the time between two science segments, the detector is either not collecting data or the collected data does not pass data quality tests} in H1 and 72 in L1 over the 20-day period. We used \textit{DeepClean} to clean each science segment, with training performed once using the first 2000\,s of the sub-segment, regardless of the length. This approach is supported by a detailed study outlined in section~\ref{sec:training}. A visualization of this strategy can be seen in Fig.~\ref{fig:retrain}.   

\begin{figure*}
    \centering
    \includegraphics[scale=0.36]{retrain.png}
    \caption{This schematic shows the training strategy used for analyzing the mock data. The grey shaded segments represent science-quality data, and the yellow indicates that a model training is performed at the beginning of each science segment. The green segments represents one-hour long inference periods where the trained model is used. That means, once a model is trained at the beginning of a science segment, all the subsequent data until the start of next science segment is cleaned using that model.}
\label{fig:retrain}
\end{figure*}



\subsection{Target noise: power-line at 60\,Hz and the side-bands}

To illustrate non-linear and non-stationary couplings, we consider the 60 Hz line of the power mains, which is modulated by low-frequency noise from LIGO's alignment sensing and control (ASC) system~\cite{Tiwari:2015ofa}. This coupling produces sidebands around the central frequency, and we use a set of witness channels that were previously used to subtract these sidebands during the third observing run (O3)~\cite{Vajente_2020}.

\subsection{Data Pre-processing}

%\ms{Avoid repetition of things from infrastructure section}

The original strain data, recorded at a rate of 16384 Hz, is downsampled to 4096 Hz for this analysis. This is because the instrumental and environmental noise we want to subtract mostly occurs at frequencies below 100\,Hz, and 4096\,Hz is sufficient for downstream analyses like detection and parameter estimation of compact binary mergers. Although \textit{DeepClean} can handle any sampling rate, a reduced rate makes training easier due to the reduced data size.

Most witness channels that are coupled to 60\,Hz power-line noise have lower sampling rates than the strain data, often below 100\,Hz or even below 10\,Hz (known as fast and slow channels). However, \textit{DeepClean} requires all input channels to have the same sampling rate. Therefore, we upsample these channels to match the strain data rate. As discussed in Sec.~\ref{sec:infra}, each channel's data is normalized independently to have zero mean and unit standard deviation. The strain data is bandpass filtered to limit the relevant frequency range for the target noise. Specifically, \textit{DeepClean} uses an 8th-order Butterworth filter to bandpass filter the data to the 55-65 Hz range. The frequency range considered here is wide enough to contain all the sidebands around 60 Hz.  


\subsection{Training}
%\ms{Avoid repetition of content from infrastructure section}

During the training process, the pre-processed data is divided into overlapping segments \textit{a.k.a} kernels\footnote{Not to be confused with the filter kernel used by the convolution operator in the CNN architecture}. These kernels are then grouped into batches, with each batch consisting of a fixed number (\texttt{batch\_size}) of kernels. For this analysis, we used a \texttt{batch\_size} of 32 with kernels that are 8\,s long and with  7\,s overlap between two kernels. This results in 25\,s of data in each batch. The entire training data of 2000\,s is then composed of 1993 overlapping kernels, which translates to a total of 80 batches. When the entire training data is passed through \textit{DeepClean} once (known as one epoch), the algorithm takes 80 iterations, with one batch taken at each iteration. At every iteration, the loss function is calculated, and backpropagated to compute the gradients, and subsequently updates the weights. In the process of  weight optimization, \textit{DeepClean} uses \textit{ADAM} optimizer\cite{AdamOptimizer} to navigate through the gradient space and minimize the loss function.

Our analysis indicates that the loss function converges in approximately 20-25 epochs during typical 60 Hz noise subtraction. This translates to roughly 1600-2000 iterations using the settings described in this example. 

%The infrastructure we use supports the technique of \textit{transfer learning}, where a previously trained model's weights can be used as an initialization for the current training. However, in our analysis, we have observed that this approach does not provide any significant improvement in the quality of the training, and therefore we have chosen not to use it.

\begin{figure*}
    \centering
    \includegraphics[width=0.495\textwidth]{ASD-plots-1251851260-2048.png}
    \includegraphics[width=0.495\textwidth]{figures/ASDR-HLL_58_62.png}
    \caption{[Left] Amplitude spectral densities (ASD) of the original and cleaned data are shown in the top (H1) and middle (L1) panels. The bottom panel shows the cleaned-to-original ASD ratio for both H1 (red) and L1 (blue). The plots are made using randomly picked 2048 seconds of MDC data from both H1 and L1. [Right] ASD ratios computed over the 20-day period of MDC data for H1 (upper) and L1 (middle and lower). Each point on the x-axis represents 256\, s of data starting from there on and the y-axis shows the minimum (blue), maximum (red) and the mean (orange) of the ASD ratio from the [55, 65] Hz band. For L1, due to quality issues (see the descussion in the text), the analysis is repeated with a narrower frequency band;z [58, 62] Hz which is shown in the bottom panel while the middle panel shows the results obtained with [55, 65] Hz.}
    \label{fig:asdr-mdc}
\end{figure*}

\subsection{Cleaning and post-processing}\label{sec-cleaning}


%To clean the data, we pre-process it by down-sampling, normalizing, and band-passing it, following the same procedure used during training. 
Unlike in training, we do not necessarily have to perform cleaning on overlapping kernels because, given a set of trained weights, the predictions for a certain data segment are always the same and do not benefit from averaging over overlapping kernels. However, when performing bulk offline analysis of thousands of seconds of data, it is inevitable to clean the long data segment after splitting into batches of shorter segments, due to memory constraints.

In addition, CNN architecture underweights the edges of the segments by design, which can lead to artifacts at the kernel edges. These artifacts get enhanced during the bandpassing step in the post-processing, and they can also spread to samples farther from the edges. To prevent these edge effects, we apply Hann windows to the predictions from overlapping kernels and employ an averaging procedure before they are band-passed.

For the offline analysis, we perform inference on 3600\,s-long (1 hour) chunks of data, using a  model that is trained at the beginning of the science segment, as previously described.



\subsection{Performance: Improvements in the noise spectral density}

To assess the quality of noise regression, we compared the ASD of the cleaned strain to the original strain in the frequency band of 55-65 Hz using ASD ratio as a metric. The ASD ratio was computed on 2048\,s of data from both H1 and L1 data, and the resulting plot (Fig.~\ref{fig:asdr-mdc}, left panel) showed a well-subtracted peak at 60\,Hz and its sidebands.  The right panel in Fig.~\ref{fig:asdr-mdc} shows the ASD ratio computed over the 20 days of MDC data. Each point on the x-axis (in units of seconds) represents the 256\, s data starting from that second onwards. For each x value, there are three y values, which are the minimum, maximum, and the mean of the ASD ratio of that particular 256\, s. For example, at each point, there will be an ASD ratio curve similar to the bottom panel on the left. The \textit{mininum} will represent the subtraction achieved at the 60 Hz peak. The \textit{maximum} is plotted with the intention of capturing ASD ratio that goes above 1, \textit{i.e.} any noise that is contributed by \textit{DeepClean}. The \textit{mean} is meant to showcase the overall subtraction in the band including the sidebands.   

In the top right panel, we have the ASD ratios from H1 noise subtraction. the maximum stays around 1, the \textit{mean} and \textit{minimum} below 1 consistently over the 20 days. This indicates a quality subtraction.  On the other hand, for L1 subtraction in the middle right panel, we notice that the \textit{maximum} of ASD ratios are well above one for many segments. These peaks in the ASD ratios are understood to be happening at 56\, Hz and 64\, Hz while the exact reason is not well understood. It can be a data quality issue either in the strain or the witness channels, leading to poorly converged models of the neural networks. We repeated the analysis by narrowing down the  frequency band to $58-62$\, Hz such that the frequencies of noisy peaks  (56\,Hz and 64\, Hz) are excluded from the band. The results are shown in the bottom right panel. It shows that the unwanted features are filtered out by appropriately narrowing down the frequency band of the analysis.    




==> sec-infrastructure.tex <==

\begin{figure*}
    \centering
    \includegraphics[scale=0.36]{workflow.png}
    \caption{The top diagram illustrates the \textit{DeepClean} architecture and the workflow. \textit{DeepClean} takes timeseries data from multiple witness channels as input and runs it through a fully convolutional autoencoder. The autoencoder has four convolution layers for downsampling and four transpose-convolution layers for upsampling. After each layer, batch normalization and a tanh activation function are applied. Finally, an output convolutional layer generates the one-dimensional noise prediction. The flowchart at the bottom depicts a typical training workflow for \textit{DeepClean}. The ADAM optimizer is employed to minimize the loss function by navigating through the gradient space.}
\label{fig:workflow}
\end{figure*}



\section{The \textit{DeepClean} infrastructure}
\label{sec:infra}

The \textit{DeepClean} architecture has been described in detail in \cite{Ormiston:2020ele}. In this section, we provide a brief overview of the algorithm. The strain readout from an interferometer, $h(t)$,  can be represented as the sum of a possible astrophysical signal $s(t)$ and the detector noise $n(t)$, such that $h(t) = s(t) + n(t)$.

The goal of \textit{DeepClean} is to minimize the noise $n(t)$ to enable the detection of the astrophysical signal at the highest possible signal-to-noise ratio (SNR). While some noise sources are fundamental and cannot be eliminated, others can be removed with the help of witness sensors~\cite{2020PhRvD.102f2003B}. We can classify the noise into two categories: \textit{witnessed} and \textit{non-witnessed} noise. The environmental and instrumental processes that contribute to the witnessed noise $n_w(t)$ are monitored by a set of channels denoted as ${w_i(t)}$, as discussed in \cite{Ormiston:2020ele}. Mathematically, the noise contributed by these channels can be expressed as an output of some activation function $\mathcal{F}$, \textit{i.e.}, $n_w(t) = \mathcal{F}({ w_i(t)})$.

In general, the activation function $\mathcal{F}$ involves non-linear and non-stationary couplings, particularly in gravitational-wave interferometers. \textit{DeepClean} is a convolutional neural network that encodes this activation function using trainable weights $\vec{\theta}$. Thus, we can express the neural network as 
\begin{equation}
    n_w(t) = \mathcal{F}({ w_i(t)}; \vec{\theta}).
\end{equation}

The \textit{DeepClean} architecture was designed to be a symmetric auto-encoder that has four downsampling layers (convolution) and four upsampling layers (transpose convolution). 
The input layer has a flexible dimensionality to match the sampling frequency and number of witness channels in the input data. the first downsampling layer is designed to have 8 channels (features) with the same sampling frequency as in the input data. Each sucessive layer downsample the data by a factor 2 and increases the number of features by a factor 2, meaning that the latent vector has 64 features. 
The four up-sampling layers halves the number of features and doubles the sampling frequency at each layer, thereby regaining the same dimensionality as the input data. An output convolutional layer is then applied to map the data into a one-dimensional time series of noise prediction. At each layer, convolution or transpose convolution is followed by batch normalization and a {\it tanh} activation function to improve the model's generalization ability. A schematic diagram of the \textit{DeepClean} architecture, along with a flowchart of a typical \textit{DeepClean} workflow, is presented in Fig.~\ref{fig:workflow}. 

The weights $\vec{\theta}$ are trained using the gradient descent algorithm~\cite{2016arXiv160904747R} by minimizing an appropriate loss function. In the case of \textit{DeepClean}, the loss function is defined as the ratio of the noise spectrum of the cleaned strain to the original strain, summed over all frequency bins within the analysis bandwidth $[f_{min}, f_{max}]$:
% \begin{equation}
% J = \frac{1}{f_{max}-f_{min}} \int_{f_{min}}^{f_{max}} \sqrt{\frac{S_r(f)}{S_h(f)}} df. 
% \end{equation}
\begin{equation}
J = \frac{1}{N} \sum_{i=1}^N \sqrt{\frac{S_r^{(i)}}{S_h^{(i)}}}
\label{eq:loss-function}
\end{equation}
Here, $S_r^{(i)}$ is the power spectral density (PSD) of the residual strain at $i^{th}$ frequency bin after subtracting $n_w(t)$. Likewise, $S_h^{(i)}$ is the PSD of the original strain at $i^{th}$ bin before subtracting $n_w(t)$. 

%%in the most general form, is defined as a weighted sum of a frequency-domain and a time-domain metrics, 
%\begin{equation}
% J = w_{asd}\, J_{asd} + w_{mse}\, J_{mse} %+ w_{edge}\, J_{edge}
%\label{eq:loss-function}
%\end{equation}
%where, $J_{asd}$ is the  and $J_{mse}$ is the mean-squared error in the time-domain strain, {\it i.e.,} the mean of the squared amplitudes of the cleaned time series. The weight parameters $w_{asd}$ and $w_{mse}$ can be chosen based on what metric should be weighted up or down in training the network. One could add additional terms to the loss function appropriately if one aims to improve any specific features in the noise regression process (as we discuss later on in section~\ref{}).  

Prior to processing with \textit{DeepClean}, both the strain and witness time-series are pre-processed by normalizing the time-series to ensure they have zero mean and unit variance. The strain data is further bandpass filtered to the frequency range of interest $[f_{min}, f_{max}]$. The pre-processed data is then input into the trained \textit{DeepClean} to predict the noise contamination. To prevent boundary artifacts, predictions are made on 8\,s segments with 4\,s overlaps. These overlapping noise predictions are then combined after applying \textit{Hann} windows to improve the prediction quality.

Subsequently, the predicted noise is band-pass filtered to $[f_{min}, f_{max}]$ to exclude any frequencies outside this range. After reversing the normalization steps, the predicted noise is subtracted from the original strain, yielding the cleaned strain.

In the following sections, we will use a mock data challenge to evaluate performance of \textit{DeepClean} and to conduct validation tests.

==> sec-intro.tex <==
\section{Introduction} \label{sec:intro}

The current network of ground-based laser interferometers, consisting of advanced LIGO ~\cite{AdLIGO,ligoHarry_2010} and advanced Virgo ~\cite{AdVIRGO} have facilitated the detection of approximately one hundred gravitational wave (GW) events from coalescing compact binaries consisting of neutron stars and/or black holes~\citep{GWTC3,Nitz:2021zwj,Olsen:2022pin}. In the third observing run (referred to as O3), LIGO Livingston (L1), LIGO Hanford (H1)  and Virgo (V1) had a sensitive median range for detecting binary neutron stars (BNS) of approximately 133\,Mpc, 115\,Mpc and 51 \,Mpc, respectively~\citep{GWTC3}. The fourth observing run, referred to as O4, has been officially started in May 2023, with recent technological upgrades and the addition of a fourth detector, KAGRA (K1)~\citep{kagraPhysRevD.88.043007,Som2012}. The range of the anticipated detection of binary neutron stars in O4 is expected to be 160-190\,Mpc for Advanced LIGO, 90-120\,Mpc for Advanced Virgo, and 1-10\,Mpc for KAGRA~\citep{OSD}.


Upgrades in technology have improved the sensitivity of interferometers by reducing fundamental noise sources such as thermal and quantum fluctuations~\citep{Cahillane:2022pqm,DaAr2021}. However, environmental and instrumental processes also contribute to the noise in the interferometer strain. The presence of such noise can reduce the sensitivity of the detectors to astrophysical transient signals~\cite{LIGO:2021ppb,2021CQGra..38b5016S}, in particular, sources without well-known theoretical models (e.g., supernovae)~\citep{Riles_2013}. Noise regression methods are used to remove these contaminants, typically by identifying their origin~\cite{Tiwari:2015ofa}. Gravitational-wave interferometers are equipped with auxiliary \textit{witness} sensors or channels to independently monitor these processes in addition to the strain channel~\cite{2021CQGra..38n5001N}. Identifying the couplings that exist between these witness channels is the key in estimating their contribution to the strain and removing them. However, there are thousands of witness channels tracking different noise sources, and non-linear couplings between them may result in noise that is challenging to identify using standard filtering techniques such as Wiener filtering~\citep{Vas2001,Say2003,Davis:2018yrz,LIGOScientific:2019hgc}.


The developments of machine learning neural networks have significantly enhanced our capability of noise regression in the interferometer strain data. This includes the recent deep learning algorithms that are developed to subtract non-linear and non-stationary couplings originating from instrumental and environmental sources~\citep{BiBl2013,ZeCo2017,PhysRevD.95.104059,Vajente_2020,Ormiston:2020ele,Yu:2021swq}. These algorithms have successfully removed noise couplings such as the 60\,Hz power-line noise and their sidebands, which arise from the non-linear coupling of the strain with instrumental control systems. However, these deep learning noise regression algorithms have thus far been demonstrated primarily in high latency, or \textit{offline}, analysis scenarios, where time-series data of several hours are analyzed long after they were originally recorded.


Multi-messenger astronomy, where gravitational-wave sources are followed up for their counterparts in the electromagnetic spectrum and neutrinos, is one of the most promising aspects of gravitational-wave observations~\citep{Abbott:2016blz,AbEA2017b}. Detecting electromagnetic counterparts that fade quickly after the gravitational-wave detection, such as $\gamma$-ray bursts and x-rays from binary neutron star mergers, requires sending out low-latency alerts to trigger follow-up observations across electromagnetic frequencies~\citep{Metzger:2016pju,Cannon:2011vi,LIGOScientific:2019gag,Sachdev:2020lfd,Chu:2020pjv,Yu:2021vvm}. Ground-based detectors are still below their designed sensitivities at lower frequency ranges (below 60\,Hz)~\citep{Abbott:2016xvh,aLIGO:2020wna}, indicating the potential for substantial improvements in the capability of sending pre-merger (or early-warning) alerts by performing low-latency noise regression at low frequencies. Even incremental improvements in the sensitive distances can lead to significant improvements in the number of detections, which scale as the cube of the distance (proportional to the volume). These improvements could result in the detection of compact binary mergers that would not have otherwise been identified at low latency.


Performing low-latency  (\textit{a.k.a} online) noise regression poses significant computational challenges compared to offline regression. To not become the dominant source of latency in the release of alerts, a low-latency noise regression should produce cleaned strain with the overall delay not more than a couple of seconds. Ref.~\cite{Gunny:2021gne} discussed in detail how to meet  such computational demands in low latency, by employing the \textit{as-a-service} computing paradigm~\citep{Krupa:2020bwg,Wang:2020fjr} into the context of gravitational-wave data analysis, in order to leverage hardware accelerators (such as GPUs) and other heterogeneous computing resources.


In this paper, we demonstrate and validate the application of \textit{DeepClean}~\cite{Ormiston:2020ele} infrastructure on gravitational wave strain data from LIGO Hanford and LIGO Livingston. \textit{DeepClean} is a deep learning convolutional neural network algorithm for noise regression in gravitational-wave strain. \textit{DeepClean} targets those noise that are environmental or technical\footnote{Technical noise, \textit{a.k.a} control noise, usually refers to the noise generated by the apparatus that control the optics in the interferometer} in origin and can be tracked independently with witness sensors. We perform a mock data challenge (MDC) to demonstrate the effectiveness of \textit{DeepClean} as a production pipeline for low-latency and high-latency noise regression applications. 

%and  non-linear, broadband noise in the 10–30 Hz band, contributed by the instrument control systems and modulated by slow-moving channels. The low-frequency noise is one of the main limiting factors of our ability to detect intermediate-mass binary black holes which merge at low frequencies. 


This paper is organized as follows:
Section~\ref{sec:infra} provides a concise overview of the DeepClean architecture and the end-to-end infrastructure.
Section~\ref{sec-MDC} presents the details of our mock data challenge.
In section~\ref{sec:inference}, we delve into the application of \textit{DeepClean} on our mock data and present the corresponding performance metrics.
Section~\ref{sec:offline-O3} demonstrates the validation tests performed using astrophysically motivated metrics, including detection and parameter estimation.
Section~\ref{sec:dc-online} focuses on the feasibility of utilizing \textit{DeepClean} for low-latency noise regression.
Finally, section~\ref{sec:conclusions} concludes the study and discusses future prospects.

==> sec-online.tex <==


\section{Feasibility Study for Low-Latency Deployment of \textit{DeepClean} }\label{sec:dc-online}

To perform noise subtraction in real-time, we must employ a different approach from the offline analysis outlined in the previous section. The offline analysis involved dividing the data into chunks of 3600\,s, predicting noise on overlapping kernels of 8\,s, and then combining them after applying window functions (see section~\ref{sec:inference} for more details). This approach necessitates having a substantial amount of data available at once, enabling the creation of overlapping 8\,s kernels. In contrast, the online analysis aims to clean the data as soon as it becomes available and make it accessible to low-latency search pipelines downstream of \textit{DeepClean}. Therefore, we need a different workflow and strategy for the online version of \textit{DeepClean}. A fully functional model of online \textit{DeepClean} complemented with the \textit{Inference-as-a-service} model will be presented in a future publication. Here, we discuss the key differences that separate it from the offline model, the issues it raises, and some preliminary figures of merit. 

%In the DeepClean workflow, the uncleaned strain time-series as well as the witness time-series are first pre-processed (bandpassing, centering and normalization) fed to the \verb|pytorch.DataLoader| object as batches of overlapping kernels. Typically, in an offline analysis, a typical batch contains 32 kernels of 8s duration, though these numbers can be conveniently changed to fit to the available memory and the number of witness channels used in the analysis. DeepClean subtraction is performed on these overlapping kernels which are then combined together after applying 'Hann' window to each kernel, before being post-processed (un-centering, un-normalizing and bandpass again to filter contents that got added into the noise outside the desired frequency band). A typical offline cleaning sends 4096s of data together and they all are treated in this way and performs very well. 

\subsection{Edge effects}

The need to develop a new strategy arises from \textit{edge effects}, which occur when the noise prediction quality deteriorates towards the edges of a kernel. Fig.~\ref{fig:edge-effects} shows that the first and last approximately 0.5\,s of a 4\,s kernel are susceptible to noisy spectral features. The width of each 4\,s segment along the vertical axis shows the difference between the online and offline predictions. The offline prediction is made on a 128\, second longer segment in which the 4 seconds shown are far from the edges. 
To mitigate these effects, \textit{DeepClean} uses overlapping  kernels and Hann windows to give more weight to the center of each kernel. This approach has been found to work well for offline cleaning. For online cleaning, our aim is always to clean the 1\,s segment that is recorded most recently. Even if we divide the 1\, s data into shorter overlapping kernels, there are no data available to overlap with the very last kernel and hence the edges can not be fully suppressed.   

The reduction in quality at the edges of the kernel can be attributed to the natural tendency of CNN architectures to discard information at the edges of input data. This is particularly relevant in \textit{DeepClean}, where we employ filter kernels of size 7 and strides of 2, resulting in the features at the edges being captured at a lower level compared to those at the middle of the kernel during convolution. For example, a sample from the middle is captured four times by the sliding filter, while a sample at the edge is only captured once. While \textit{DeepClean} attempts to alleviate this issue by using zero-padding of size 3 at the edges, the edges are still  captured only three times with this padding size. Increasing the padding size could be a potential solution, but it could lead to array size problems since the padding size is also constrained by the input-output sample size matching.


% what is written below is what we thought as a possible reason earlier, however we don't have the same opinion now. 
%We expect that part of the reason for why the edges are affected could be the way the network learns the features in the data. We have allowed the network to train the weights by minimizing the ASD, which is computed from overlapping kernels. As we train with at least a few hundreds of seconds of data, a ``good enough'' ASD can be achieved even when the edges are affected, by virtue of windowing. Alternative choices of loss functions and windowing could perhaps solve this issues, although our preliminary attempts were unsuccessful and this will be the subject of future work.   

\begin{figure*}
    \centering
    \includegraphics[scale=0.86]{sliding-window-model.pdf}
    \caption{The diagram shows how \textit{DeepClean} will be used for low-latency (online) denoising. The figure compares the online and offline predictions, both normalized, for 4-second duration segments. The offline prediction for the same segment is extracted from the middle of a 128-second-long prediction. The difference bars indicate that the predictions differ only at the edges, which are less than a second long. To avoid edge effects, \textit{DeepClean} is applied to 8 seconds of data, consisting of 6 seconds from the past and 1 second from the future, in addition to the 1 second of target data. This is done for every 1 second frame, and the wait for a future frame causes an additional 1 second of latency. After the prediction, everything except the 1 second target data is discarded from the 8-second segment and written to disk as cleaned frames, ready for downstream analyses.}
\label{fig:edge-effects}
\end{figure*}


\subsection{A working model for $\sim 1s$ latency}

While ongoing work aims to comprehensively address edge effects, a simple modification to the workflow can mitigate the issue in the meantime. This resolution comes at the cost of a latency of approximately 1 second. To ensure that the quality of our online analysis matches that of our offline analysis, we employ a 4-second kernel that includes 2 seconds of data before and 1 second after the 1-second target segment. The additional data ensures that the target segment is located in the center of the kernel. The DeepClean is then applied on the 4-second kernel, and the 1-second target segment is extracted for analysis. A cartoon depicting this is shown in Fig.~\ref{fig:edge-effects}.

As the affected edges are not exactly 1\,s in length, we can select a part of the output that is closer to the edge where we aggregated the future data. This edge, where future data is aggregated, is referred to as the aggregation latency. Fig.~\ref{fig:asdr-latency-online} displays a scatter plot with the achieved ASD ratio on the x-axis and the overall latency\footnote{The \textit{overall latency} is the term referred to as the latency in producing the cleaned frames \textit{w.r.t} the time when the original frame became available. It is comprised of the time taken to load the data, perform subtraction, and write the output frame to disc, in addition to the aggregation latency.} on the y-axis, for different aggregation latencies. It is evident that the subtraction quality gets better by allowing higher aggregation latencies as shown by the reduced ASD ratios in the graph. 



%\begin{figure*}
%    \centering
%    \includegraphics[scale=0.7]{online-working-model}
%    \caption{Demonstration of a low-latency pipeline working model. Due to the edge effects discussed in the text, %For every 1\,s frame, \textit{DeepClean} is applied to 8\,s of data with 6\,s from past and 1\,s from future, in addition to the 1\,s of target data to avoid the target being on the edges. The wait for a future 1\,s frame causes 1\,s of additional latency. After the prediction is made, everything except the 1\,s target are discarded from the 8\,s segment and written to disk as cleaned frames ready for downstream analyses.}
%    \label{fig:dc-online-working-model}
    
%\end{figure*}


\begin{figure}
    \centering
    %\includegraphics[scale=0.25]{latency_online.pdf}
    %\includegraphics[scale=0.25]{ASDR_online.pdf}
    \includegraphics[scale=0.25]{ASDR_vs_latency_online.pdf}
    \caption{Scatter plot showing the latency vs quality trade-off.  The overall latency referred to here is the time taken by DeepClean to produce the output strain after the raw strain is made available. The ASD (amplitude spectral density) ratio on the x-axis is computed from every 32\,s of the data. The three different colors shows the different aggregation latencies. Notably, the quality of the ASD ratio improves with higher aggregation latency, at the cost of increased overall latency.}
    \label{fig:asdr-latency-online}
    
\end{figure}



==> sec-pe.tex <==


\subsection{Parameter estimation of coalescing binaries}

After applying a denoising pipeline, it is critical to perform parameter estimation (PE) of the underlying astrophysical signals as a validation test. This serves two purposes: firstly, to ensure that the regression analysis has not affected the original signals and, secondly, to assess any improvement in the credible intervals of the estimated parameters resulting from noise-subtraction. In this study, we focus only on the first purpose since the noise subtraction of 60 Hz alone may not yield any notable improvement in the credible interval. 

To perform this test, we selected injections from our MDC dataset based on their coalescence frequencies. The coalescence frequency, also known as the frequency of the last stable circular orbit of a binary evolution, is given by $f_{lso} = (6^{3/2}\,\pi\, m)^{-1}$ Hz, where $m=m_1+m_2$ is the total mass of the binary in the observer frame. We pick only those injections whose $f_{lso}$ lies between 55\,Hz and 70\,Hz. We choose this frequency range because our target noise is around 60\,Hz  and signals with a peak frequency around 60\,Hz would demonstrate the most significant scientific benefits. We found 258 BBH injections that satisfy this source criterion.


The literature contains well-described methods for estimating parameters from gravitational-wave signals, and there are standard analysis pipelines available that use stochastic samplers \citep{Veitch:2014wba,Ashton:2018jfp}. For our analysis, we utilized tools from the \textit{Bilby} \citep{Ashton:2018jfp} Bayesian library. We ran the \textit{Dynesty} sampler~\cite{2019S&C....29..891H} to sample from a 15-dimensional parameter space that included the luminosity distance, two mass parameters, six spin parameters, the time and phase of the binary coalescence, and four angles defining the binary's sky-location and orientation relative to the line of sight.  

Out of the 258 injections, only 84 events met the minimum signal-to-noise ratio criterion of 4 at both detectors, confirming their detection and indicating the potential for reliable parameter estimation. Additionally, we did encounter sporadic instances where the cleaned data was noisier than the original data. We subsequently excluded these affected segments from our analysis and we were then left with 78 injections for our PE study. In order to address this issue for practical online setups, we need to incorporate validation tests to ensure that the outputs of the \textit{DeepClean} algorithm are not noisier than the original. If the \textit{DeepClean} output is found to be noisier, one needs to replace them with the original data as a baseline solution. More involved approaches to resolve this issue would include increasing the cadence of training.


We conducted parameter estimation (PE) on both the denoised and original strain data, and compared the results. 
%Additionally, we performed PE on data cleaned using the online inference pipeline, utilizing the same trained model as for the offline inference. 
In Fig.~\ref{fig:corner-3param}, we present 3D posteriors of the luminosity distance and two mass parameters obtained from one of the 258 injections we analyzed. The posteriors from the cleaned data (orange) are consistent with those of the original data (blue). This indicates that the noise regression analysis did not introduce any unwanted noise components or remove any spectral features from the signal itself. The same is true even if \textit{DeepClean} is trained on data that has injections, as shown in the green curve.   

%Accurate estimation of the power spectral density (PSD) used in likelihood computation is crucial in Bayesian parameter estimation. Typically, the PSD is estimated from a long stretch of neighboring data, several hundred seconds in length, that do not contain any signal. However, due to the closely packed nature of our injections, it can be challenging to find a long enough segment without a signal to estimate the PSD. If an astrophysical or injected signal is present in the PSD estimation segment, the PSD may inaccurately represent the noise in the analysis data. To address this, we first estimated PSDs from data without injections, and then repeated the parameter estimation analyses with PSDs estimated from injected data. We found that our results were not notably different between the two PSD estimation methods, as shown in Fig.~\ref{fig:corner-3param}.
%{\color{blue} We use the same PSD files estimated without any injections. The difference shown in Fig.~\ref{fig:corner-3param} is the cleaning model of DeepClean.}

Fig.~\ref{fig:pp-plots-offline} displays p-p plots for the fifteen parameters from the 78 events, showing excellent agreement between the p-p plots before \textit{DeepClean} (left) and after \textit{DeepClean} (right). This observation is essential as it validates the safety of the underlying astrophysical signals when the \textit{DeepClean} algorithm is applied. This result demonstrates that the algorithm does not harm the underlying astrophysical signals and hence supports the reliability of the analysis. 



%We find that the p-p plots for the original and cleaned data are consistent, as we found in the corner plot. In some cases, we do see that the p-p plot for both original and cleaned data are deviating from the expected behaviour. In other words, there are some events, for which some of the injected parameters are recovered far from the posterior credible regions, for example, luminosity distance. Since this analysis is done with low latency data that has a number of non-gaussian artifacts such as glitches, either the analysis segment can have some additional features or as the more likely case, the PSD segment will have some non-Gaussianity in it leading to biased PSD estimations. Since the Bayesian PE is highly sensitive to the differences in the statistical properties of the noise and the PSD, the PE can get biased as we observed in this case. We have also noticed that the biased PSDs are often happening in one of the two detectors, however, it serves as sufficient to bias the combined PE results.   

%In Fig.~\ref{fig:pe-CI}, we show the reduction in the error bars of the posterior distributions. Figure shows the ratio of the symmetric 90\% credible intervals of the posteriors from the cleaned data to that from the original data. If there is a significant improvement in the posteriors, then we would expect the histograms to center below 1. However, all of our histograms are centered around 1 indicating that there is no notable improvement in the error bars particularly due to the subtraction of the 60 Hz powerline and sidebands. The fact that the error bar ratio is distributed on either sides of unity may be attributed to the variations from the sampling uncertainties. 

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/corner_plot_3parameter.png}
    \caption{ %{(\color{blue} Update with event 76)} 
    Corner plot showing the posteriors of the mass parameters and the luminosity distance before and after the subtraction of the 60 Hz power-line and their side-bands using \textit{DeepClean}}
    \label{fig:corner-3param}
\end{figure}



\begin{figure*}
    \centering
    \includegraphics[scale=0.53]{figures/pp-plot-org-mdc-78-events.png}
    \includegraphics[scale=0.53]{figures/pp-plot-dc-mdc-78-events.png}

    \caption{P-P plots generated from the parameter estimation studies of 78 binary black hole injections, comparing the results before and after the application of the \textit{DeepClean} algorithm for offline noise subtraction. The x-axis represents the credible interval, while the y-axis shows the fraction of injections recovered within that interval. These P-P plots are used to validate whether the injected parameters, after noise regression, can be recovered within the statistical uncertainty limits. As seen in the figure, the parameter recovery after \textit{DeepClean} is at least as good as, if not better than, that achieved prior to applying the algorithm. The P-values included in the plots are derived from the Kolmogorov-Smirnov test, which quantifies the degree to which the credible interval distributions differ from the expected distributions.}
    \label{fig:pp-plots-offline}
\end{figure*}


% \begin{figure*}
%     \centering
%     \includegraphics[scale=0.3]{figures/CI_width_frac.png}
%     \caption{Figure showing the improvement in the 90\% credible intervals of the posteriors estimated from the data after DeepClean analysis.}
%     \label{fig:pe-CI}
% \end{figure*}








%More-or-less the sectino from "Safety checks" Ideally, present statistical quantities that reflect the posterior improvements on m1, m2 (m chirp/q), RA, Dec, d L, i.e., the most crucial parameters for low latency EM followup.

%For example, delta-X (x=mass, q, RA, Dec, d L) of peak values, or 90\% CL intervals with and without DeepClean.

%Ideally, delta-X should be consistent with systematic errors (aka, calibration, assuming we use the same WF family) and 90\% CL intervals from DeepClean should be fully contained within the non-DeepClean ones.


%\subsection{Safety checks for the online analysis}
%In section~\ref{sec:offline-O3}, we have already demonstrated that the underlying astrophysical signals remains unaffected after the data is run through the offline \textit{DeepClean} pipeline. However, that may not guarantee that the same would hold for the online analysis as well, as the cleaned time series samples are  extracted differently from the offline analysis. 
%Since the analysis included every 1\,s cleaned frames being cropped off from the 8\,s cleaned frames and then combined together (particularly from the vicinity of the deteriorated kernel edges), it would be prudent to ensure that no spectral content is lost or added into in the process.
%For this reason, we test a few BBH signals injected into the data and ensure they can be well recovered from the data that are cleaned. We also compare the improvements in the credible intervals before and after subtracting the noise power. 

%We perform three analyses here .... (add the details and updated figures)



%segments with only two parameters; for computational purposes, we sample chirp mass and the luminosity distance as unknown parameters, while the rest of the parameters are assumed to be known and therefore fixed to their true values. While this assumption is motivated by the computational expense, we expect this test is sufficient to demonstrate that \textit{DeepClean} does no harm, as any changes in the signal shape or the amplitude will reflect as biases in either the chirp mass or the luminosity distance, or both. 


%Fig.~\ref{fig:pe-offline} (left) shows the histograms of the median estimates of the chirp mass (top left) and the luminosity distance (top right). Four traces represent 1) analysis of cleaned data with signals injected prior to the cleaning, 2) analysis of cleaned data with signals injected after the cleaning, 3) analysis of unclean data with signals injected, and 4) the injected distribution of parameters.  The plots clearly indicates consistency between the injected and recovered signal parameters, showing that the \textit{DeepClean}  does not remove any signal content from the strain data. (explain more). 

%Fig.~\ref{fig:pe-offline}  (right) shows the histograms of the 90\% credible intervals from the three PE analyses described above. It is evident that the credible intervals improve by the noise regression. More quantitatively, we find that the credible intervals shrink by xx\% on an average. (The figure is not yet ready!)




==> sec-training.tex <==

\subsection{A case study for training DeepClean at low latency}
\label{sec:training}

% The process of DeepClean training, like training any NN, works based on the choices made for several parameters that governs how the network learns the correlations between the strain and witness data. The parameters include, for example, the learning rate and weight decay of the gradient descent algorithm, in addition to the loss function model parameters and some external parameters such as duration of the data used for training and re-training frequency etc. In this work, primarily limited by the hardware resources, we restrict our focus onto the effects of 1) the duration of the data, 2) selection of segments and the frequency of training (or the cadence for re-training), and  3) choice of loss function models and its weight parameters. A more thorough and exhaustive study, exploring all possible training dependencies is currently being done with the help of the recently-developed Inference-as-a-Service model which enables fast executions of DeepClean workflows on hardware-accelerators such as GPUs. However, we deffer these studies for a future publication. As a prototype, again, we have used only the 60 Hz noise subtraction for the training studies in this paper. 

% For the offline DeepClean analyses, the first decision to make is on the segment selection for training, precisely, where to choose the segments from and of what duration. Our analyses have shown that a duration less than 1000\,s is sub-optimal for most cases, while we do not gain significantly in terms of subtraction quality by increasing the training duration beyond $\sim$\,2000\,s. 
% We show this in Fig.~\ref{fig:training-vs-duration} where ASD ratio distributions for different training duration are plotted. Based on this, we have chosen 4096\,s for training in all of our production analyses (discussed in earlier section). 

% Regarding the selection of segments and frequency of training, there are various possible alternatives one could go with: 1) train on exactly the same data as the target segment (on-segment training), 2) to train on a segment that is nearest to the target segment 3), to train once in every lock stretch, and 4) to train once during several lock-losses.

% In Fig.~\ref{fig:training-seg-selection}, we show the ASD ratio histograms with all these alternatives.
% We find the following from our analyses:
% \begin{itemize}

% 	\item The best ASD ratio results are obtained when the network is trained on the target segments. This is expected as it allows the network to learn all the features in the data including those which are specific to the target segments.  However, these improvements are not significantly higher compared to scenarios (1) and (2).  
	
% 	\item There is added benefit to train once in every lock stretch, compared to training just once in an observing run. However, we do not see any significant difference between training once in a lock stretch and training from every nearby segment.  
	
% 	\item The results suggest that the noise features changes subtly over the course of time, especially while the detector is in lock after a lock-loss. However, the features change very little over the course of a lock stretch. 
	
% \end{itemize}

\begin{figure}
    \centering
    \includegraphics[scale=0.6]{figures/training_cadence.pdf}
    \caption{The figure underscores the significance of periodically retraining the neural network, \textit{deepClean}. It presents two traces for each detector: one representing the cleaned strain data from day 1 (solid line) and the other displaying the cleaned strain from day 20 (dashed line), derived from our 20-day MDC dataset. The horizontal axis depicts the GPS time of the training data, with an initial time conveniently set to zero. Meanwhile, the vertical axis represents the Amplitude Spectral Density Ratio (ASDR). Notably, there is an observed increase in ASDR when the training data is selected from a segment further away from the cleaning data, particularly noticeable in H1. In contrast, the disparity in ASDR between training and cleaning data is less prominent in L1 over this 20-day period. Overall, the figure emphasizes the importance of regular retraining to ensure optimal performance and accurate data cleaning.}
    \label{fig:training-vs-asdr-hist}
    
% Location: https://jupyter.ligo-wa.caltech.edu/user/muhammed.saleem/lab/workspaces/auto-2/tree/deepClean/deepclean/explore_training/modified_training_monthly_stats.ipynb
\end{figure}



To enable real-time gravitational wave data cleaning, it is necessary to train and validate the machine learning model in short timescales. Unlike offline analysis where there is sufficient time to optimize and fine-tune the trained model, online cleaning requires that the model be trained quickly and validated frequently. This is because the noise features in the data are generally non-stationary, and the noise coupling that \textit{DeepClean} once learned could change after a certain time, making it necessary to have new models periodically trained on the most recent data.

To explore this in detail, we conducted a case study using the 20 days of MDC data. We trained the model once for each science segment, resulting in a total of 47 trained models for H1 and 72 for L1 over the 20 days. We then took two examples of inference data, one from day 1 and the other from day 20, and cleaned them with all the models available. Fig.~\ref{fig:training-vs-asdr-hist} shows the ASD ratio results on the y-axis and the time (from the 20 days) where the model is trained on the x-axis. The solid line represents the data from day 1, and the dashed line represents the data from day 20, for both the detectors. 
%used these models to clean data that were closer to the respective training dataset as well as those that were far away from them. Our results show that the trained models become sub-optimal over time, with a change in the ASD ratio as we go away from the time of the training dataset.
%To illustrate this, we 

It is observed that the ASD ratio changes as we move away from the time of the training dataset, particularly in H1 data. For instance, the day 1 data has an ASD ratio below 0.6 when trained with data from day 1, 2, or 3, but the ASD ratio goes above 0.6 when the training dataset is from day 20. The same observation is true for cleaning the data from day 20, which is best cleaned with the model trained on day 20.

Although this study indicates that trained models become sub-optimal over time, we noticed that it does not happen over the timescale of minutes or hours, but rather changes over the timescale of days. In L1, we do not notice any significant change in the ASD ratio over time, which may be an indication that the coupling features in L1 are rather stationary. Overall, our observations emphasize that there is enough time for training and validating a model that is trained at low latency.

It should be noted that these observations are based on our cleaning of 60\,Hz powerline and sidebands. The timescale over which the coupling features change will also depend on the coupling itself. For example, a different coupling in a different frequency range, can be highly non-stationary and would require model retraining at a higher cadence. Fortunately, our production deployment of \textit{DeepClean} is highly compute-efficient due to leveraging the GPU resources and hence capable of training once every 30 minutes or less. The details of that is differed for a later publication.

